THE-Tree: Can Tracing Historical Evolution Enhance Scientific Verification and Reasoning?

Large Language Models (LLMs) are accelerating scientific idea generation, but rigorously evaluating these numerous, often superficial, AI-generated propositions for novelty and factual accuracy is a critical bottleneck; manual verification is too slow. Existing validation methods are inadequate: LLMs as standalone verifiers may hallucinate and lack domain knowledge (our findings show 60% unawareness of relevant papers in specific domains), while traditional citation networks lack explicit causality and narrative surveys are unstructured. This underscores a core challenge: the absence of structured, verifiable, and causally-linked historical data of scientific evolution.To address this,we introduce \textbf{THE-Tree} (\textbf{T}echnology \textbf{H}istory \textbf{E}volution Tree), a computational framework that constructs such domain-specific evolution trees from scientific literature. THE-Tree employs a search algorithm to explore evolutionary paths. During its node expansion, it utilizes a novel "Think-Verbalize-Cite-Verify" process: an LLM proposes potential advancements and cites supporting literature. Critically, each proposed evolutionary link is then validated for logical coherence and evidential support by a recovered natural language inference mechanism that interrogates the cited literature, ensuring that each step is grounded. We construct and validate 88 THE-Trees across diverse domains and release a benchmark dataset including up to 71k fact verifications covering 27k papers to foster further research. Experiments demonstrate that i) in graph completion, our THE-Tree improves hit@1 by 8% to 14% across multiple models compared to traditional citation networks; ii) for predicting future scientific developments, it improves hit@1 metric by nearly 10%; and iii) when combined with other methods, it boosts the performance of evaluating important scientific papers by almost 100%.

==> tex/checklist.tex <==

\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The Abstract and Section 1 show our paper's contributions and scopes.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We fully discuss the limitations in Section 5.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  This paper focuses on providing results based on metrics. The related results are presented in Section 4.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We disclose the implementation details of reproducing the results of this paper in Appendix A and Appendix B.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Due to proprietary considerations currently under review, we have decided to release the code at a later stage. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We disclose the implementation details of reproducing the results of the paper in Appendix A and B. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Performing multiple repetitive experiments in order to compute error bars is labor-intensive and has significant overhead for the large language model development.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All LLM-based module implemented through API-driven inference methods.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our research follows the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We fully discuss the potential social impacts in Section 7.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: To facilitate the safe release of data, we provide a detailed description of the dataset construction process in Section 3 and Appendix A, along with the evaluation results in Section 4.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide reasonable references for the datasets and models used in Section 4 and Appendix A.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the relevant documentation in Section 4 and the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This research does not involve any crowdsourcing experiments or human subjects research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA meNAs that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: LLMs are integral to our core methodology in multiple critical components. These uses of LLMs are essential to our framework's operation and are thoroughly described in Section 3.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> tex/discussion.tex <==
\section{Discussion}
% 中文注释：讨论

% % 5.1 主要发现与意义
% \subsection{Main Findings and Implications}
% 中文注释：5.1 主要发现与意义
The THE-Tree framework, as demonstrated through our experiments, successfully constructs verifiable, causally-linked technology evolution trees from scientific literature.
% 中文注释：正如我们的实验所证明的，THE-Tree框架成功地从科学文献中构建了可验证的、具有因果关联的技术演化树。
This addresses a critical gap identified in the Introduction and Related Work: the lack of structured, reliable, and machine-readable representations of scientific history.
% 中文注释：这解决了引言和相关工作中指出的一个关键差距：缺乏结构化的、可靠的、机器可读的科学史表示。
By moving beyond the limitations of noisy citation networks and unstructured surveys, THE-Tree provides a more robust, fact-based foundation for understanding the intricate dynamics of scientific progress.
% 中文注释：通过超越充满噪声的引文网络和非结构化综述的局限性，THE-Tree为理解科学进步的复杂动态提供了更稳健、基于事实的基础。

The key significance lies in its ability to represent historical lineage and validated causal dependencies explicitly.
% 中文注释：其关键意义在于它能够明确地表示历史谱系和经过验证的因果依赖关系。
This explicit structure enables deeper reasoning about how ideas build upon one another, which traditional bibliometric methods struggle to capture with the same level of granularity and verified causality.
% 中文注释：这种明确的结构使得能够更深入地推理思想是如何相互构建的，而传统文献计量方法难以用相同的粒度和经过验证的因果关系来捕捉这一点。
Furthermore, the successful application of THE-Tree in downstream tasks like future node prediction and graph completion underscores its practical utility. It demonstrates that modeling the validated evolutionary process can enhance predictive accuracy and provide a superior representation of knowledge structure compared to simpler network models.
% 中文注释：此外，THE-Tree在未来节点预测和图补全等下游任务中的成功应用突显了其实用价值。它表明，对经过验证的演化过程进行建模可以提高预测准确性，并提供比简单网络模型更优越的知识结构表示。

Our work pioneers large-scale, verifiable causal reasoning about technology evolution. By tracing validated dependency chains, THE-Tree enables comparative analyses of evolution rates and patterns of influence across diverse scientific fields.
% 中文注释：我们的工作开创了关于技术演进的大规模、可验证的因果推理。通过追踪经过验证的依赖链，THE-Tree使得能够对不同科学领域的演化速率和影响模式进行比较分析。
For instance, quantifying the average time lag for method transfer from a foundational field like computer vision to an applied domain like medical imaging is made more robust when based on explicitly validated evolutionary steps rather than mere citation proximity or keyword co-occurrence.
% 中文注释：例如，量化方法从计算机视觉等基础领域转移到医学影像等应用领域的平均时间滞后（例如，[在此处插入具体时间，如果结果确认，例如2.7年]），当基于明确验证的演化步骤而非仅仅是引文邻近性或关键词共现时，会更加稳健。
This deeper, causally-informed understanding of "how science moves" can inform science policy, guide research strategy, and foster interdisciplinary collaboration more effectively.
% 中文注释：这种对"科学如何发展"的更深刻、基于因果的理解，可以更有效地为科学政策提供信息，指导研究策略，并促进跨学科合作。
In essence, THE-Tree provides not just a new way to visualize scientific history, but a computable framework for reasoning about its structure and dynamics, crucial for navigating the scientific landscape and guiding future discovery.
% 中文注释：从本质上讲，THE-Tree不仅提供了一种可视化科学史的新方法，而且提供了一个用于推理其结构和动态的可计算框架，这对于在科学领域中导航和指导未来发现至关重要。

% % 5.2 创新应用
% \subsection{Innovative Applications}
% % 中文注释：5.2 创新应用
% The structured and validated nature of THE-Tree opens up several novel application possibilities beyond direct research evaluation:
% % 中文注释：THE-Tree的结构化和经过验证的特性开启了超越直接研究评估的几种新颖应用可能性：

% \textbf{Informed Funding Decision Support:} Traditional metrics for assessing technology maturity often lack deep historical context. THE-Tree enables the development of more nuanced indicators like a Technology Maturity Index (TMI), derived from a technology's validated position within its evolutionary trajectory, its connectivity, and temporal dynamics. This offers richer insights than simple age or citation counts, potentially identifying foundational technologies for emerging fields.
% % 中文注释：知情的资助决策支持：评估技术成熟度的传统指标往往缺乏深厚的历史背景。THE-Tree使得开发更细致的指标成为可能，例如技术成熟度指数（TMI），该指数源自技术在其演化轨迹中的已验证位置、其连接性和时间动态。这提供了比简单的年龄或引文计数更丰富的见解，可能识别出新兴领域的基础技术。
% % Equation for TMI (Optional): %
% % \begin{equation} %
% % \text{TMI}(i) = f(\text{Position}(i), \text{Connectivity}(i), \text{Dynamics}(i)) %
% % \end{equation}

% \textbf{Structured Educational Tooling:} Understanding the prerequisite structure of knowledge is key for effective learning. THE-Tree can generate subject learning path maps (e.g., "essential papers from linear regression to GNNs") grounded in actual, validated evolutionary dependencies. These reflect the demonstrable historical build-up of ideas, offering more robust learning trajectories than paths based on co-occurrence or subjective opinions.
% % 中文注释：结构化教育工具：理解知识的先决条件结构是有效学习的关键。THE-Tree可以生成基于实际的、经过验证的演化依赖关系的学科学习路径图（例如，"从线性回归到GNNs的必读论文"）。这些路径反映了思想的可证明的历史积累过程，提供了比基于共现或主观意见的路径更稳健的学习轨迹。

% \textbf{Strategic Enterprise Innovation Navigation:} Identifying genuine "white space" for innovation requires mapping the technological landscape. THE-Tree allows systematic identification of technology combination gaps – unexplored intersections between distinct trajectories. A Gap Score could assess potential based on the strength of existing/absent validated links and historical trajectories, providing a reliable basis for R&D planning.
% % 中文注释：战略性企业创新导航：识别真正的创新"空白地带"需要绘制技术图景。THE-Tree允许系统地识别技术组合的空白——不同轨迹之间未经探索的交叉点。空白得分（Gap Score）可以基于现有/缺失的已验证链接的强度和历史轨迹来评估潜力，为研发规划提供可靠的基础。
% % Equation for GapScore (Optional): %
% % \begin{equation} %
% % \text{GapScore}(i, j) = g(\text{Similarity}(i, j), \text{ConnectionStrength}(i, j), \text{Potential}(i, j)) %
% % \end{equation}

% These examples illustrate how a computable, verifiable history of science, as provided by THE-Tree, can translate into practical tools for researchers, educators, policymakers, and industry strategists.
% % 中文注释：这些例子说明了由THE-Tree提供的可计算、可验证的科学史如何转化为研究人员、教育工作者、政策制定者和行业战略家的实用工具。


% \jiyaocomm{Moved to here from related work} \textbf{Positioning THE-Tree}
% % 中文注释：THE-Tree的定位
% In contrast to the aforementioned approaches, THE-Tree makes several distinct contributions to address the identified gaps.\\
% % 中文注释：与上述方法相比，THE-Tree为解决已识别的差距做出了几个独特的贡献。
% (1) It focuses on constructing explicit \textbf{technology evolution trees} that represent historical lineage and validated causal dependencies between scientific contributions, moving beyond general citation networks or static, entity-focused knowledge graphs.\\
% % 中文注释：(1) 它专注于构建明确的“技术演化树”，这些树代表科学贡献之间的历史谱系和经过验证的因果依赖关系，超越了通用的引文网络或静态的、以实体为中心的知识图谱。
% (2) It incorporates a rigorous TVCV methodology with RA-NLI to ensure the verifiability, logical coherence, and factual grounding of the identified evolutionary relationships in scientific literature. This directly addresses the noise and lack of explicit causality often found in traditional bibliometric networks and the potential for ungrounded assertions from LLMs.\\
% % 中文注释：(2) 它整合了严格的“思考-表达-引用-验证（TVCV）”方法论以及“检索增强自然语言推断（RA-NLI）”，以确保所识别的演化关系在科学文献中的可验证性、逻辑连贯性和事实基础。这直接解决了传统文献计量网络中常见的噪声和缺乏明确因果关系的问题，以及LLM可能做出无根据断言的风险。
% (3) While leveraging LLM reasoning (via SGT-MCTS, and within TVCV) for exploring and structuring this historical evolution, THE-Tree ensures that outputs are \textbf{systematically grounded in and validated against verifiable literature evidence}, rather than relying on the LLM's standalone declarative knowledge.\\
% % 中文注释：(3) 尽管利用LLM的推理能力（通过自引导时序蒙特卡洛树搜索SGT-MCTS以及在TVCV内部）来探索和结构化这种历史演化，THE-Tree确保输出被系统地锚定在可验证的文献证据上并据此进行验证，而不是依赖LLM独立的陈述性知识。
% By providing this structured, verifiable, and causally-linked history, THE-Tree directly tackles the critical data gap that hinders robust, history-based evaluation of scientific ideas and provides a more solid, fact-based foundation for guiding AI-driven scientific discovery.\\
% % 中文注释：通过提供这种结构化的、可验证的、具有因果关联的历史，THE-Tree直接解决了阻碍对科学思想进行稳健的、基于历史的评估的关键数据空白，并为指导AI驱动的科学发现提供了更坚实、基于事实的基础。


==> tex/newmethod.tex <==
\
\sout{\section{Methodology}}
{\color{blue}\section{THE-Tree as Scientific Verifier}}
% 中文注释：章节标题修改：Methodology -> THE-Tree 作为科学验证器

\sout{\subsection{Conceptual Framework: Representing Scientific Progress as a Technology Evolution Tree}}
% 中文注释：\sout{3.1. 概念框架：将科学进步表征为技术演化树}
{\color{blue}\subsection{THE-Tree: A Structured Representation of Scientific Evolution}}
% 中文注释：新增小节 3.1：THE-Tree：科学演化的结构化表示

{\color{blue}
% 中文注释： addressing the need for a better way to represent scientific evolution...
The pursuit of scientific discovery is increasingly aided by AI, yet verifying the novelty and validity of numerous AI-generated or human-conceived hypotheses presents a significant bottleneck, as highlighted in our Abstract and Introduction. Traditional methods like citation networks lack the necessary semantic depth, offering only noisy and superficial links, while LLMs as standalone verifiers can hallucinate or miss crucial domain knowledge. This underscores the urgent need for a structured, verifiable, and causally-linked representation of scientific evolution.
% 中文注释：科学发现的探索日益得到人工智能的辅助，然而，正如我们在摘要和引言中所强调的，验证大量由AI生成或人类构思的假说的新颖性和有效性构成了一个重大瓶颈。传统方法如引文网络缺乏必要的语义深度，仅提供充满噪声和表面的链接，而大型语言模型作为独立验证器可能会产生幻觉或缺乏关键领域知识。这凸显了对结构化、可验证且具有因果关联的科学演化表示的迫切需求。

To address this challenge, we introduce the \textbf{THE-Tree (Technology History Evolution Tree)}.
% 中文注释：为应对这一挑战，我们引入了THE-Tree（技术历史演化树）。
In a THE-Tree, each scientific paper is conceptualized as a \textbf{node}.
% 中文注释：在THE-Tree中，每篇科学论文被概念化为一个节点。
Each node encapsulates rich metadata crucial for understanding the paper's context, contribution, and significance. This information typically includes the paper's title, abstract, authors, publication venue, and publication year. Furthermore, each node \(v\) is associated with a computationally derived importance score \(S_v\), reflecting its relevance and impact within the specific domain, as will be detailed in Section~\ref{sec:auto_construction_importance_score}.
% 中文注释：每个节点都封装了理解论文背景、贡献和重要性的关键元数据。这些信息通常包括论文的标题、摘要、作者、发表机构和发表年份。此外，每个节点v都关联一个计算得出的重要性评分S_v，反映其在特定领域内的相关性和影响力，具体细节将在章节~\ref{sec:auto_construction_importance_score}中阐述。

The \textbf{edges} in a THE-Tree represent the \textbf{historical, inferential, and evolutionary relationships} between these paper nodes.
% 中文注释：THE-Tree中的边代表了这些论文节点之间的历史性、推理性及演化性关系。
}
\sout{Scientific ideas and technological advancements evolve through historical progression and logical connections, which can be structured as a tree-like directed graph. In this representation, individual scientific papers serve as nodes, and the historical, inferential, and evolutionary relationships between these papers constitute the edges.}
% 中文注释：\sout{科学观点和技术的发展遵循历史演进和逻辑关联，可以被构建为一个类树的有向图结构。在此表示中，单篇科学论文作为节点，而论文之间的历史推演和演化关系则构成边。}
{\color{blue}
Unlike traditional citation networks, where an edge might merely indicate a citation without specifying the nature of the relationship, edges in THE-Tree are imbued with deeper semantic meaning. They are constructed to signify how one paper (or the ideas and technologies presented therein) causally contributes to, logically enables, or provides an essential foundation for the advancements detailed in a subsequent, connected paper.
% 中文注释：与传统引文网络不同（传统网络中的边可能仅表示一次引用而未指明关系性质），THE-Tree中的边被赋予了更深层次的语义。它们旨在表明一篇论文（或其中提出的思想和技术）如何因果地贡献于、逻辑上促成或为后续连接论文中详述的进展提供必要基础。
This distinction is critical. While traditional citation links are valuable, they are often too simplistic or noisy (e.g., perfunctory citations, negative citations, or citations to general background rather than specific conceptual building blocks) to accurately map the nuanced, multi-step evolution of scientific ideas. Our methodology, further detailed in Section~\ref{sec:auto_construction_edges} (referring to SGT-MCTS and TVCV parts), therefore focuses on identifying and establishing edges that reflect substantive intellectual lineage and direct technological dependence, aiming to filter out superficial connections and capture the true pathways of innovation.
% 中文注释：这种区别至关重要。虽然传统的引用链接有其价值，但它们往往过于简单化或充满噪声（例如，敷衍的引用、反面引用，或引用一般背景而非特定的概念构建模块），难以准确描绘科学思想细致入微、多步骤的演化过程。因此，我们的方法论（在章节~\ref{sec:auto_construction_edges}中进一步详述，指SGT-MCTS和TVCV部分）专注于识别和建立能够反映实质性学术传承和直接技术依赖的边，旨在滤除表面连接并捕捉真实的创新路径。

The primary purpose of constructing and utilizing THE-Trees is to provide a \textbf{structured, verifiable, and causally-linked historical tapestry of scientific evolution} for specific domains.
% 中文注释：构建和利用THE-Tree的主要目的是为特定领域提供一个结构化的、可验证的、具有因果关联的科学演化历史图谱。
This detailed, graph-based representation serves as a robust knowledge scaffold. It allows new scientific propositions—whether generated by humans or AI—to be situated within an explicit, evidence-backed evolutionary context. By tracing connections and analyzing pathways within the THE-Tree, we can more rigorously assess a new idea's novelty (i.e., does it genuinely extend or diverge from known paths?), its factual consistency with established knowledge, and its potential impact, thereby addressing the limitations of standalone LLM evaluators and often unstructured narrative surveys. THE-Tree thus facilitates a more evidence-based approach to scientific idea validation.
% 中文注释：这种详细的、基于图的表示构成了一个强大的知识支架。它使得新的科学主张——无论是人类还是AI产生的——能够被置于一个明确的、有证据支持的演化背景中。通过在THE-Tree中追溯连接和分析路径，我们可以更严格地评估一个新思想的新颖性（即，它是否真正扩展或偏离了已知路径？）、其与既有知识的事实一致性及其潜在影响，从而克服了独立LLM评估器和通常非结构化的叙述性综述的局限性。因此，THE-Tree促进了一种更基于证据的科学思想验证方法。
}

\sout{Our approach formulates the construction of such a THE-Tree as an optimization problem. The goal is to identify paths through scientific literature that maximize a composite reward, reflecting the importance of the constituent nodes (papers) and the coherence of the evolutionary process they represent:}
% 中文注释：\sout{我们的方法将构建这样一个技术历史演化树（THE-Tree）表述为一个优化问题，旨在找到科学文献中的路径，以最大化一个复合奖励，该奖励反映了构成路径的节点（论文）的重要性以及它们所代表的演化过程的连贯性：}
\sout{\begin{equation}}
\sout{\max_{\text{Path}} \left( \sum_{v \in \text{Path}} S(v) + R_{\text{gen}} + R_{\text{attr}} \right),}
\sout{\end{equation}}
\sout{where \(S(v)\) is the importance score of a node (paper) \(v\), \(R_{\text{gen}}\) is the generation process reward reflecting the coherence of the path, and \(R_{\text{attr}}\) is the attribution process reward validating the link between connected nodes. This objective is pursued using the SGT-MCTS algorithm, detailed below.}
% 中文注释：\sout{其中S(v)是节点（论文）v的重要性得分，R_gen是反映路径连贯性的生成过程奖励，R_attr是验证相连节点间链接的归因过程奖励。此目标通过下文详述的SGT-MCTS算法实现。}
\sout{Furthermore, we propose a straightforward method for leveraging the constructed THE-Tree for technological retrospection. Detailed explanations are provided in Appendix~\ref{app:the_tree_retrospection_method} and will not be further elaborated within this methodology section.}
% 中文注释：\sout{此外，我们提供了一种利用已构建的THE-Tree进行技术回顾的简单方法。由于这并非本文的核心贡献，详细内容请参阅附录~\ref{app:the_tree_retrospection_method}，方法论部分将不再赘述。}

{\color{blue}\subsection{Leveraging THE-Tree for Scientific Idea Verification}}
% 中文注释：新增小节 3.2：利用THE-Tree进行科学观点验证
{\color{blue}
Once a THE-Tree, with its richly annotated nodes and semantically meaningful edges, is constructed for a specific scientific domain, it serves as a powerful instrument for the verification and contextualization of new scientific ideas or papers. We propose a straightforward yet effective methodology to utilize THE-Tree for this purpose, enabling the retrospection of relevant historical evolutionary paths for a given input scientific paper, \(P_{in}\), defined by its title \(T_{in}\) and abstract \(A_{in}\). This approach provides critical context by situating new research within established knowledge frameworks, thereby aiding in the assessment of its novelty and potential contribution.
% 中文注释：一旦为特定科学领域构建了具有丰富注释节点和语义意义边的THE-Tree，它便成为验证和情境化新科学思想或论文的强大工具。我们提出了一种直接而有效的方法来利用THE-Tree实现此目的，即对给定的输入科学论文（\(P_{in}\)，由其标题\(T_{in}\)和摘要\(A_{in}\)定义）进行相关历史演化路径的回溯。这种方法通过将新研究置于已建立的知识框架内来提供关键背景，从而有助于评估其新颖性和潜在贡献。

The core steps of this verification and retrospection process are as follows:
% 中文注释：此验证和回溯过程的核心步骤如下：
\begin{enumerate}
    \item \textbf{Initialization}: This methodology assumes access to:
    % 中文注释：1. 初始化：此方法论假定可以访问：
    \begin{itemize}
        \item A collection of pre-computed THE-Trees \(\{G_k\}\), where each \(G_k = (V_k, E_k)\) corresponds to a specific scientific topic \(Topic_k\). Nodes \(v \in V_k\) represent scientific papers with attributes such as publication year \(Y_v\), title \(T_v\), abstract \(A_v\), and an importance score \(S_v\), as defined in Section 3.1. Edges \(e \in E_k\) signify directed evolutionary relationships, capturing inferential and developmental dependencies.
        % 中文注释：一组预先计算的THE-Tree \(\{G_k\}\)，其中每个\(G_k = (V_k, E_k)\)对应一个特定的科学主题\(Topic_k\)。节点\(v \in V_k\)代表科学论文，具有如3.1节定义的发表年份\(Y_v\)、标题\(T_v\)、摘要\(A_v\)和重要性评分\(S_v\)等属性。边\(e \in E_k\)表示有向的演化关系，捕捉推断和发展依赖。
        \item A Large Language Model (LLM) for semantic tasks such as similarity assessment and topic matching.
        % 中文注释：一个用于语义任务（如相似性评估和主题匹配）的大型语言模型（LLM）。
    \end{itemize}

    \item \textbf{Topic Space Identification}: For the input paper \(P_{in}\), a set of \(N_T\) most relevant topics, \(\mathcal{T}_{P_{in}} = \{Topic_1, \dots, Topic_{N_T}\}\), is identified from the available THE-Tree topics. This involves prompting an LLM with \(T_{in}\), \(A_{in}\), and the list of all THE-Tree topic names to determine the most appropriate THE-Tree(s) for situating \(P_{in}\).
    % 中文注释：2. 主题空间识别：对于输入论文\(P_{in}\)，从可用的THE-Tree主题中识别出一组\(N_T\)个最相关的主题\(\mathcal{T}_{P_{in}} = \{Topic_1, \dots, Topic_{N_T}\}\)。这包括使用\(T_{in}\)、\(A_{in}\)和所有THE-Tree主题名称列表提示LLM，以确定最适合定位\(P_{in}\)的THE-Tree。

    \item \textbf{Candidate Path Origination in Relevant THE-Trees}: For each identified topic \(Topic_k \in \mathcal{T}_{P_{in}}\) and its corresponding THE-Tree \(G_k\):
    % 中文注释：3. 在相关THE-Tree中候选路径的起源：对于每个识别出的主题\(Topic_k \in \mathcal{T}_{P_{in}}\)及其对应的THE-Tree \(G_k\)：
    \begin{enumerate}[label=(\alph*)]
        \item Identify a candidate set of \(M_k\) recent papers \(\{v_{k,j}\} \subset V_k\) from \(G_k\) based on publication year \(Y_{v_{k,j}}\) (e.g., papers published within a certain recent time window or up to the year of \(P_{in}\) if known).
        % 中文注释：(a) 根据发表年份\(Y_{v_{k,j}}\)从\(G_k\)中识别出一组候选的\(M_k\)篇近期论文\(\{v_{k,j}\} \subset V_k\)（例如，在某个近期时间窗口内或截至\(P_{in}\)发表年份（如果已知）的论文）。
        \item Calculate a semantic similarity score \(Sim(P_{in}, v_{k,j}) \in [0,1]\) between the input paper \(P_{in}\) (using its title and abstract) and each candidate \(v_{k,j}\) (using its stored title and abstract) using an LLM or other embedding-based techniques.
        % 中文注释：(b) 使用LLM或其他基于嵌入的技术，计算输入论文\(P_{in}\)（使用其标题和摘要）与每个候选论文\(v_{k,j}\)（使用其存储的标题和摘要）之间的语义相似度得分\(Sim(P_{in}, v_{k,j}) \in [0,1]\)。
        \item Select the top \(N_S\) papers from these candidates, denoted \(\mathcal{S}_k = \{v^*_{k,1}, \dots, v^*_{k,N_S}\}\), that exhibit a similarity score \(Sim(P_{in}, v^*_{k,l}) \geq \theta_{sim}\), where \(\theta_{sim}\) is a predefined minimum similarity threshold. These papers \(v^*_{k,l}\) serve as terminal nodes (or "entry points") for backward path tracing within the THE-Tree, representing the most closely related established works to \(P_{in}\).
        % 中文注释：(c) 从这些候选项中选择前\(N_S\)篇论文，表示为\(\mathcal{S}_k = \{v^*_{k,1}, \dots, v^*_{k,N_S}\}\)，这些论文的相似度得分\(Sim(P_{in}, v^*_{k,l}) \geq \theta_{sim}\)，其中\(\theta_{sim}\)是预定义的最小相似度阈值。这些论文\(v^*_{k,l}\)作为在THE-Tree内进行反向路径追溯的终端节点（或“入口点”），代表与\(P_{in}\)最密切相关的已确立工作。
    \end{enumerate}

    \item \textbf{Historical Path Retrospection}: For each selected terminal paper \(v^*_{term} \in \mathcal{S}_k\) in graph \(G_k\):
    % 中文注释：4. 历史路径回溯：对于图\(G_k\)中每个选定的终端论文\(v^*_{term} \in \mathcal{S}_k\)：
    \begin{itemize}
        \item A historical path \(Path_{k,l} = (v_1, v_2, \dots, v_n=v^*_{term})\) is constructed by iteratively selecting predecessors. This path traces the lineage of \(v^*_{term}\) backward through the THE-Tree.
        % 中文注释：通过迭代选择前驱节点来构建历史路径\(Path_{k,l} = (v_1, v_2, \dots, v_n=v^*_{term})\)。此路径通过THE-Tree反向追溯\(v^*_{term}\)的谱系。
        \item Starting from \(v_{curr} = v^*_{term}\), the predecessor \(v_{pred}^*\) is chosen from the set of all predecessors \(Pred(v_{curr})\) (i.e., nodes from which an edge points to \(v_{curr}\)) according to the lexicographical optimization that prioritizes strong evolutionary links and historical relevance:
        % 中文注释：从\(v_{curr} = v^*_{term}\)开始，根据优先考虑强演化链接和历史相关性的词典优化，从所有前驱节点集合\(Pred(v_{curr})\)（即有边指向\(v_{curr}\)的节点）中选择前驱节点\(v_{pred}^*\)：
        \[ v_{pred}^* = \arg\min_{v \in Pred(v_{curr}), Y_v \le Y_{v_{curr}}} ( (Y_{v_{curr}} - Y_v), -S_v ) \]
        This heuristic prioritizes the predecessor with the smallest non-negative time difference \((Y_{v_{curr}} - Y_v)\), reflecting direct chronological succession, and secondarily, the one with the highest importance score \(S_v\), indicating significant contributions. The use of node attributes \(Y_v\) (year) and \(S_v\) (importance) from the THE-Tree structure is central here.
        % 中文注释：该启发式方法优先选择具有最小非负时间差\((Y_{v_{curr}} - Y_v)\)的前驱节点，反映直接的时间顺序继承；其次选择具有最高重要性评分\(S_v\)的前驱节点，表明其重大贡献。此处核心在于使用THE-Tree结构中的节点属性\(Y_v\)（年份）和\(S_v\)（重要性）。
        \item Traversal continues backward until no valid predecessor (respecting chronological order and edge semantics) is found, a predefined maximum path length is exceeded, or a root node of the THE-Tree (a node with no predecessors in the context of this path's history) is reached. The resulting path is then presented in chronological order from the earliest paper to \(v^*_{term}\).
        % 中文注释：反向遍历持续进行，直到找不到有效的前驱节点（尊重时间顺序和边语义）、超过预定义的最大路径长度，或达到THE-Tree的根节点（在此路径历史背景下没有前驱节点的节点）。然后，生成的路径按从最早的论文到\(v^*_{term}\)的时间顺序列出。
    \end{itemize}

    \item \textbf{Path Aggregation and Presentation}: All generated paths \(\{Path_{k,l}\}\) are collected. They can be ranked based on various criteria, such as the semantic similarity score \(Sim(P_{in}, v^*_{term})\) of their terminal nodes to the input paper \(P_{in}\), the cumulative importance of nodes in the path, or the overall coherence of the path. The top \(N_P\) unique paths are selected and formatted for presentation. This presentation details the sequence of papers, their key attributes (title, year, summary of contribution derived from abstract/node info), and the nature of the connecting evolutionary relationships.
    % 中文注释：5. 路径聚合与呈现：收集所有生成的路径\(\{Path_{k,l}\}\)。可以根据各种标准对它们进行排序，例如其终端节点与输入论文\(P_{in}\)的语义相似度得分\(Sim(P_{in}, v^*_{term})\)、路径中节点的累积重要性或路径的整体连贯性。选择前\(N_P\)条唯一路径并格式化以供呈现。此呈现详细说明了论文序列、其关键属性（标题、年份、从摘要/节点信息派生的贡献摘要）以及连接演化关系的性质。
\end{enumerate}
This methodology provides a simple yet powerful way to leverage the structured knowledge within THE-Trees to verify a new scientific idea by exploring its historical context and connections to established research. The retrieved paths can highlight the foundations upon which \(P_{in}\) builds, identify potentially overlooked prior art, or help assess its incremental novelty versus a more radical departure from existing trajectories. Users can adapt this general approach based on specific analytical needs, such as modifying the LLM prompts, similarity thresholds, path selection heuristics, or the depth of retrospection.
% 中文注释：该方法论提供了一种简单而强大的方式，利用THE-Tree内的结构化知识，通过探索新科学思想的历史背景及其与既有研究的联系来进行验证。检索到的路径可以突显\(P_{in}\)所基于的基础，识别可能被忽视的先前技术，或帮助评估其相对于现有轨迹是增量式创新还是更激进的突破。用户可以根据具体的分析需求调整此通用方法，例如修改LLM提示、相似度阈值、路径选择启发式或回溯深度。
}

{\color{blue}\subsection{Automated Construction of THE-Tree}}
\label{sec:auto_construction}
% 中文注释：新增小节 3.3：THE-Tree的自动化构建
{\color{blue}
The manual construction of comprehensive and accurate THE-Trees for diverse scientific domains would be a prohibitively laborious task. Therefore, we develop a computational framework for the automated construction of THE-Trees from scientific literature. Our approach formulates this construction as an optimization problem: the goal is to identify and assemble evolutionary paths through the literature that maximize a composite reward. This reward is designed to reflect the significance of the constituent papers (nodes) and the logical coherence and evidential support of the evolutionary steps (edges) they represent:
% 中文注释：为不同科学领域手动构建全面且准确的THE-Tree将是一项极其繁重的任务。因此，我们开发了一个计算框架，用于从科学文献中自动构建THE-Tree。我们的方法将这种构建表述为一个优化问题：目标是识别并组装文献中的演化路径，以最大化一个复合奖励。该奖励旨在反映构成路径的论文（节点）的重要性以及它们所代表的演化步骤（边）的逻辑连贯性和证据支持：
\begin{equation}
\label{eq:optimization_goal}
\max_{\text{Path}} \left( \sum_{v \in \text{Path}} S(v) + R_{\text{gen}} + R_{\text{attr}} \right),
\end{equation}
% 中文注释：公式1：最大化路径的复合奖励，包括节点重要性S(v)、生成过程奖励R_gen和归因过程奖励R_attr。
where \(S(v)\) is the importance score of a node (paper) \(v\) (see Section~\ref{sec:auto_construction_importance_score} for how \(S(v)\) is determined), \(R_{\text{gen}}\) is the generation process reward reflecting the coherence of the path (how well a new node continues an existing path), and \(R_{\text{attr}}\) is the attribution process reward validating the evidential support for the link (edge) between connected nodes. This objective is pursued using a Self-Guided Temporal Monte Carlo Tree Search (SGT-MCTS) algorithm, as detailed in the pipeline stages below.
% 中文注释：其中S(v)是节点（论文）v的重要性得分（S(v)的确定方式详见~\ref{sec:auto_construction_importance_score}节），R_gen是反映路径连贯性的生成过程奖励（衡量新节点对现有路径的延续程度），R_attr是验证相连节点间链接（边）证据支持的归因过程奖励。此目标通过自引导时序蒙特卡洛树搜索（SGT-MCTS）算法实现，具体流程阶段如下所述。
}

% // ... existing code ...
\sout{\subsection{THE-Tree Construction Pipeline}}
{\color{blue}\subsubsection{THE-Tree Construction Pipeline Overview}}
% 中文注释：小节标题修改：THE-Tree Construction Pipeline -> THE-Tree Construction Pipeline Overview (3.3.1)
The construction of a THE-Tree involves several key stages, from initial data preparation to the iterative refinement of the tree structure. {\color{blue}Figure~\ref{fig:overview} provides a schematic overview of this pipeline.}
% 中文注释：THE-Tree的构建涉及几个关键阶段，从初始数据准备到树结构的迭代优化。图~\ref{fig:overview} 提供了此流程的示意图。

\begin{figure}[htb] % Consider moving this figure to a more suitable place if needed
    \centering
    \includegraphics[width=1\linewidth]{figs/overview.png}
    \caption{\textbf{THE-Tree construction overview.} (a) Extracting chunks and references from surveys to build an initial concept graph structure; (b) Generating a structured knowledge tree using the SGT-MCTS algorithm, guided by the TVCV methodology for node expansion and RA-NLI for relationship validation.
    % 中文注释：THE-Tree构建概览：（a）从综述中提取引用语句和参考文献以构建初始图结构；（b）使用SGT-MCTS算法生成结构化知识树，并通过TVCV方法进行节点扩展，通过RA-NLI进行关系验证。
}
    \label{fig:overview}
\end{figure}

\sout{\subsubsection{Dataset Construction: Initialization and Foundation}}
{\color{blue}\paragraph{Dataset Construction: Initialization and Foundation.}}
\label{sec:auto_construction_dataset}
% 中文注释：段落标题修改：Dataset Construction: Initialization and Foundation (3.3.1.1)
% 中文注释：\sout{3.2.1. 数据构建：初始化与基础。本节阐述了THE-Tree构建的数据基础，强调了从科学综述开始的重要性及其结构化处理的必要性。}
The foundation for THE-Tree construction is a structured, temporally-rich, and causally-informative dataset derived from multiple authoritative scientific surveys. These surveys, selected from diverse time periods for each topic, help mitigate recency bias and provide a broad historical perspective. The core output of this stage is an interconnected dataset comprising survey documents, identified paper nodes (from citations), concept nodes (core ideas extracted from paragraphs), and their explicit relationships. This dataset overcomes the limitations of unstructured narratives and noisy citation networks, enabling the detailed construction of technology evolution histories. Further details on this data construction pipeline are elaborated in Appendix~\ref{app:dataset_construction_details}.
% 中文注释：THE-Tree构建的基础是一个结构化的、包含时间维度且能反映因果关系的数据集，该数据集源自多篇权威的科学综述。这些针对每个主题从不同时间段挑选的综述有助于减轻新近度偏见并提供广阔的历史视角。此阶段的核心输出是一个相互关联的数据集，包含综述文档、识别出的论文节点（来自引文）、概念节点（从段落中提取的核心观点）及其明确关系。该数据集克服了非结构化叙述和噪声引文网络的局限性，为详细构建技术演化历史提供了可能。关于此数据构建流程的更多细节在附录~\ref{app:dataset_construction_details}中详述。

\sout{{\color{blue}The journey of constructing a THE-Tree begins with scientific surveys. These documents are invaluable as they encapsulate rich historical and inferential information about scientific progression, making them an ideal starting point for tracing technological evolution. % 中文注释：构建THE-Tree的起点是科学综述，因为它们包含了丰富的科学进展历史和推断信息。
However, directly utilizing raw surveys presents challenges due to their predominantly unstructured narrative format, lacking the explicit relational information needed for a computational model. % 中文注释：然而，直接利用原始综述面临挑战，因为它们主要是非结构化的叙述格式，缺乏计算模型所需的明确关系信息。
To address this, our first crucial step is to transform these surveys into a structured dataset. We strategically select surveys from diverse time periods for each topic to mitigate recency bias and capture a broader, less noisy historical perspective. % 中文注释：因此，我们首先将综述结构化，并特意挑选不同时间段的综述以减少新近度偏差，获得更全面的历史视角。
The core output of this stage is an interconnected dataset comprising survey documents, identified paper nodes (from citations within the surveys), concept nodes (core ideas extracted from paragraphs), and their explicit relationships. This structured foundation overcomes the limitations of raw narratives and noisy citation networks, enabling the detailed construction of technology evolution histories.}}
% 中文注释：\sout{此阶段的输出是一个包含综述、论文节点、概念节点及其明确关系的结构化数据集，为后续构建技术演化历史奠定了基础。}
\sout{Further details on this data construction pipeline are elaborated in Appendix~\ref{app:dataset_construction_details}.}
% 中文注释：\sout{关于此数据构建流程的更多细节在附录~\ref{app:dataset_construction_details}中详述。}


\sout{\subsubsection{Core Component: Self-Guided Temporal Monte Carlo Tree Search (SGT-MCTS)}}
{\color{blue}\paragraph{Core Component: Self-Guided Temporal Monte Carlo Tree Search (SGT-MCTS).}}
\label{sec:auto_construction_sgt_mcts}
% 中文注释：段落标题修改：Core Component: Self-Guided Temporal Monte Carlo Tree Search (SGT-MCTS) (3.3.1.2)
% 中文注释：\sout{3.2.2. 核心组件：自引导时序蒙特卡洛树搜索 (SGT-MCTS)。在结构化数据的基础上，我们采用SGT-MCTS算法来构建THE-Tree。}
With the structured dataset {\color{blue}(Section~\ref{sec:auto_construction_dataset})} as our bedrock, we employ a Self-Guided Temporal Monte Carlo Tree Search (SGT-MCTS) \cite{browne2012survey} algorithm to navigate the vast space of potential technological evolutionary paths and construct the THE-Tree. SGT-MCTS iteratively builds the tree by strategically selecting nodes for expansion, simulating potential future paths, and backpropagating rewards to update the value of explored paths (see Algorithm~\ref{alg:sgt_mcts}). The search is guided by the composite reward function introduced earlier {\color{blue}(Equation~\ref{eq:optimization_goal}: \(S(v) + R_{\text{gen}} + R_{\text{attr}}\))}, which balances node importance with path coherence and link validity.
% 中文注释：我们采用SGT-MCTS算法 \cite{browne2012survey} 来探索潜在技术演化路径的广阔空间并构建THE-Tree。该算法通过策略性选择节点进行扩展、模拟未来路径并反向传播奖励来迭代构建树。搜索过程由复合奖励函数（公式~\ref{eq:optimization_goal}）指导，平衡节点重要性、路径连贯性和链接有效性。

Central to the SGT-MCTS guidance are the node importance assessment and generation process reward:
% 中文注释：SGT-MCTS指导的核心是节点重要性评估和生成过程奖励：

\textbf{LLM-Enhanced Node Importance Assessment (\(S(v)\))}: \label{sec:auto_construction_importance_score} The importance of a paper (node \(v\)) is a weighted combination of its structural significance within the citation graph and its semantic relevance as assessed by an LLM: \(S(v) = \gamma \cdot S_{\text{graph}}(v) + (1-\gamma) \cdot S_{\text{LLM}}(v)\), where \(\gamma\) is a weighting factor. \(S_{\text{graph}}(v)\) combines multiple centrality measures (PageRank, citation count, Degree, Betweenness, Eigenvector Centrality) with dynamic weighting. \(S_{\text{LLM}}(v)\) is obtained by prompting an LLM to assess the paper's importance within the specified topic.
% 中文注释：LLM增强的节点重要性评估 (S(v))：\label{sec:auto_construction_importance_score} 论文（节点v）的重要性是其在引文图中的结构重要性与LLM评估的语义相关性的加权组合。S_graph(v)结合多种中心性度量，S_LLM(v)通过LLM评估获得。

\textbf{Generation Process Reward (\(R_{\text{gen}}\))}: This reward encourages the formation of coherent and temporally sound evolutionary paths. It is defined for a node \(v\) given a preceding path \(P_{prev}\): \(R_{\text{gen}}(v | P_{prev}) = \text{DPO}(v | P_{prev}) \cdot \text{TemporalCoherence}(v | P_{prev})\). The DPO score \cite{rafailov2023direct}, approximated by an LLM, evaluates how well node \(v\) continues the trajectory of \(P_{prev}\). The Temporal Coherence term penalizes achronological or large time gaps.
% 中文注释：生成过程奖励 (R_gen)：此奖励鼓励形成连贯且时间上合理的演化路径。它结合了评估节点v对前序路径P_prev轨迹继承程度的DPO得分 \cite{rafailov2023direct} 和惩罚非时序或大时间间隔的时间连贯性项。
\sout{The SGT-MCTS UCT formula is enhanced with LLM guidance and temporal coherence:}
% 中文注释：\sout{SGT-MCTS UCT公式通过LLM指导和时间一致性得到增强：}

\sout{{\color{blue}The selection of nodes during the SGT-MCTS process is guided by an Upper Confidence Bound 1 applied to Trees (UCT) formula \cite{kocsis2006bandit}. Our SGT-UCT variant, presented below, incorporates LLM guidance and temporal coherence to refine this selection}:}
% 中文注释：\sout{SGT-MCTS中的节点选择由UCT公式 \cite{kocsis2006bandit} 指导。我们的SGT-UCT变体整合了LLM指导和时间连贯性来进行优化选择：}
{\color{blue}The selection of nodes during the SGT-MCTS process is guided by an Upper Confidence Bound 1 applied to Trees (UCT) formula \cite{kocsis2006bandit}. Our SGT-UCT variant, presented in Equation~\ref{eq:sgt_uct}, incorporates LLM guidance and temporal coherence to refine this selection:}
% 中文注释：SGT-MCTS中的节点选择由树置信上限（UCT）公式\cite{kocsis2006bandit}指导。我们的SGT-UCT变体，如公式~\ref{eq:sgt_uct}所示，整合了LLM指导和时间连贯性以优化选择：
%

\sout{\small}
\sout{\begin{equation}}
\sout{\text{SGT-UCT}(v) = \left(\underbrace{\frac{Q(v)}{N(v)}}_{\text{cumulative reward}} + c \cdot \underbrace{\sqrt{\frac{\ln N(p)}{N(v)}}}_{\text{exploration term}} + \lambda \cdot \underbrace{\text{LLM}_{\text{priority}}(v)}_{\text{semantic priority}} \right)\cdot \text{TempCoherence}(v | P_{prev})}
\sout{\end{equation}}

\small
\begin{equation} \label{eq:sgt_uct}
\text{SGT-UCT}(v) = \left(\frac{Q(v)}{N(v)} + c \cdot \sqrt{\frac{\ln N(p)}{N(v)}} + \lambda \cdot \text{LLM}_{\text{priority}}(v)\right)\cdot \text{TempCoherence}(v | P_{prev})
\end{equation}
%
\sout{{\color{blue}In this formula, \(Q(v)/N(v)\) represents the exploitation component, which is the empirical mean reward of node \(v\) based on its past simulations, reflecting its historical performance. % 中文注释：公式中的 Q(v)/N(v) 是利用项，代表基于过去模拟的节点v的经验平均回报，反映其历史表现。
The term \(c \cdot \sqrt{\ln N(p)/N(v)}\) is the exploration component, where \(N(p)\) is the visit count of the parent node and \(N(v)\) is the visit count of the current node \(v\); this term encourages the algorithm to explore nodes that have been visited less frequently. % 中文注释：c * sqrt(ln N(p)/N(v)) 是探索项，鼓励算法探索访问频率较低的节点。
The \(\text{LLM}_{\text{priority}}(v)\) term introduces semantic guidance, representing the priority of node \(v\) as assessed by an LLM, steering the search towards thematically relevant advancements. % 中文注释：LLM_priority(v) 项引入语义指导，代表LLM评估的节点v的优先级，引导搜索朝向主题相关的进展。
Finally, the entire expression is modulated by \(\text{TempCoherence}(v | P_{prev})\), which acts as a filter to ensure that the selected path maintains chronological consistency. % 中文注释：最后，整个表达式由 TempCoherence(v | P_prev) 调节，作为确保所选路径保持时间一致性的过滤器。
The constants \(c\) and \(\lambda\) are hyperparameters balancing these components.}}
{\color{blue}In this formula (Equation~\ref{eq:sgt_uct}), \(Q(v)/N(v)\) is the exploitation component (empirical mean reward of node \(v\)). The term \(c \cdot \sqrt{\ln N(p)/N(v)}\) is the exploration component, encouraging visits to less explored nodes (\(N(p)\) is parent visit count, \(N(v)\) is current node visit count). \(\text{LLM}_{\text{priority}}(v)\) injects semantic guidance from an LLM. The entire expression is modulated by \(\text{TempCoherence}(v | P_{prev})\) to enforce chronological path consistency. Constants \(c\) and \(\lambda\) are balancing hyperparameters.}
% 中文注释：在此公式（公式~\ref{eq:sgt_uct}）中，\(Q(v)/N(v)\)是利用项（节点v的经验平均回报）。\(c \cdot \sqrt{\ln N(p)/N(v)}\)是探索项，鼓励访问探索较少的节点（\(N(p)\)是父节点访问次数，\(N(v)\)是当前节点访问次数）。\(\text{LLM}_{\text{priority}}(v)\)注入来自LLM的语义指导。整个表达式由\(\text{TempCoherence}(v | P_{prev})\)调节，以强制路径按时间顺序保持一致。常数\(c\)和\(\lambda\)是平衡超参数。

We also implement reward-sensitive exploration where the exploration coefficient \(c(t)\) increases with the average reward, encouraging broader exploration in promising regions.
% 中文注释：我们还实现了奖励敏感的探索，其中探索系数c(t)随平均奖励增加而增加，以鼓励在有前景的区域进行更广泛的探索。

\sout{\subsubsection{Node Expansion Method: Think-Verbalize-Cite-Verify (TVCV) Methodology}}
{\color{blue}\paragraph{Node Expansion Method: Think-Verbalize-Cite-Verify (TVCV) Methodology.}}
\label{sec:auto_construction_tvcv}
% 中文注释：段落标题修改：Node Expansion Method: Think-Verbalize-Cite-Verify (TVCV) Methodology (3.3.1.3)
% 中文注释：\sout{3.2.3. 节点扩展方法：Think-Verbalize-Cite-Verify (TVCV) 方法论。SGT-MCTS通过TVCV方法论进行节点扩展，即添加新的论文节点并建立它们之间的连接。}
Node expansion within SGT-MCTS, the process of adding new paper nodes and establishing connections {\color{blue}(edges with rich semantic meaning as discussed in Section 3.1)}, is performed using our novel Think-Verbalize-Cite-Verify (TVCV) methodology (see Algorithm~\ref{alg:tvcv_expansion}). This process leverages an LLM to systematically generate, ground, and validate new nodes (potential technological advancements) and their links within the tree:
% 中文注释：SGT-MCTS内的节点扩展（添加新论文节点并建立连接（如3.1节所讨论的具有丰富语义意义的边）的过程）采用我们新颖的TVCV方法论（见算法~\ref{alg:tvcv_expansion}）。该过程利用LLM系统地生成、锚定和验证树中的新节点（潜在技术进步）及其链接：
\begin{itemize}[leftmargin=*]
    \item \textbf{Think:} The LLM generates candidate technological advancements or scientific contributions that could logically follow from the current path history and domain knowledge.
    % 中文注释：Think：LLM根据当前的路径历史和领域知识，生成候选的技术进步或科学贡献。
    \item \textbf{Verbalize:} The LLM summarizes these generated ideas into concise statements or propositions that represent potential new nodes.
    % 中文注释：Verbalize：LLM将生成的想法总结为简洁的陈述或命题，代表潜在的新节点。
    \item \textbf{Cite:} For each summarized proposition, the LLM retrieves or identifies specific supporting scientific literature (i.e., existing paper nodes from the dataset or newly found papers) that grounds the proposed advancement, thereby proposing a potential link between an existing paper node and a new one.
    % 中文注释：Cite：针对每个总结的命题，LLM检索或识别具体的支持性科学文献（即来自数据集的现有论文节点或新发现的论文），为提议的进步提供依据，并由此提出一个现有论文节点与新节点之间的潜在链接。
    \sout{\item \textbf{Verify:} The proposed relationship between the current path and the new cited node, along with the node itself, is rigorously validated for logical consistency, causal coherence, and temporal soundness. This step centrally involves the RA-NLI mechanism described next.}
    \sout{\item \textbf{Verify:} {\color{blue}The proposed relationship (edge) between the current path's terminal node and the newly cited paper node, along with the relevance of the new node itself, is rigorously validated. This crucial step ensures the factual and logical soundness of the link, and is performed by the RA-NLI mechanism.}}
    {\color{blue}\item \textbf{Verify:} The proposed relationship (edge) between the current path's terminal node and the newly cited paper node, along with the relevance of the new node itself, is rigorously validated for logical consistency, causal coherence, and temporal soundness. This crucial step, ensuring the factual and logical soundness of the link, is performed by the RA-NLI mechanism described in Section~\ref{sec:auto_construction_ranli}.}
    % 中文注释：Verify：对当前路径末端节点与新引用的论文节点之间的提议关系（边）以及新节点本身的相关性进行严格验证，确保其逻辑一致性、因果连贯性和时间合理性。这个关键步骤确保了链接的事实和逻辑健全性，并由章节~\ref{sec:auto_construction_ranli}中描述的RA-NLI机制执行。
\end{itemize}

\sout{\subsubsection{Relationship Validation: Retrieval-Augmented Natural Language Inference (RA-NLI) Mechanism}}
{\color{blue}\paragraph{Relationship Validation: Retrieval-Augmented Natural Language Inference (RA-NLI) Mechanism.}}
\label{sec:auto_construction_ranli} 
\label{sec:auto_construction_edges}
% 中文注释：段落标题修改：Relationship Validation: Retrieval-Augmented Natural Language Inference (RA-NLI) Mechanism (3.3.1.4)
% 中文注释：\sout{3.2.4. 关系验证：检索增强的自然语言推断 (RA-NLI) 机制。RA-NLI机制用于在TVCV过程中验证论文节点之间生成的关系的逻辑和事实一致性。}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/nli_frame.png}
    \caption{\textbf{Overview of RA-NLI process.} This figure illustrates the RA-NLI process, including citation existence verification, document retrieval, and semantic relation assessment using NLI and LLM, which forms the core of the \textit{Verify} step in TVCV and the $R_{\text{attr}}$ calculation.
    % 中文注释：该图展示了RA-NLI过程，包括引文存在性验证、文献检索以及使用NLI和LLM进行的语义关系评估，这是TVCV中"Verify"步骤和R_attr计算的核心。
    }
    \label{fig:nli_frame}
\end{figure*}
The critical \textit{Verify} step of the TVCV methodology {\color{blue}(Section~\ref{sec:auto_construction_tvcv})}, and the basis for the attribution process reward (\(R_{\text{attr}}\)) {\color{blue}in Equation~\ref{eq:optimization_goal}}, is performed by our Retrieval-Augmented Natural Language Inference (RA-NLI) mechanism. RA-NLI is designed to rigorously assess the causal and logical coherence of the evolutionary link (edge) proposed between a parent node (e.g., \(v_{\text{parent}}\)) and a newly cited child node (\(v\)),
% 中文注释：TVCV方法论中关键的"Verify"步骤（章节~\ref{sec:auto_construction_tvcv}），以及归因过程奖励（R_attr）（公式~\ref{eq:optimization_goal}中）的基础，是由我们的检索增强自然语言推断（RA-NLI）机制执行的。RA-NLI旨在严格评估在父节点（例如v_parent）和新引用的子节点（v）之间提议的演化链接（边）的因果和逻辑连贯性。
\begin{equation}R_{\text{attr}}(v_{\text{parent}} \to v) =   \text{RA-NLI}(s_{\text{parent}}, s_v)\end{equation}
This mechanism (illustrated in Figure~\ref{fig:nli_frame}) integrates embedding-based retrieval to fetch relevant contextual passages from the cited documents, followed by fine-grained Natural Language Inference using a specialized model (\(f_{\text{NLI}}\)) to determine if the textual description of the child node (\(s_v\)) is entailed, contradicted by, or neutral with respect to the parent node's description (\(s_{\text{parent}}\)) and supporting evidence. An LLM-based verifier (\(f_{\text{LLM}}\)) further refines ambiguous cases. This ensures semantic soundness and high fidelity for the identified evolutionary relationships, forming the backbone of the THE-Tree's verifiability.
% 中文注释：该机制（如图~\ref{fig:nli_frame}所示）集成了基于嵌入的检索，以从被引文献中获取相关的上下文段落，然后使用专门的模型（f_NLI）进行细粒度的自然语言推断，以确定子节点的文本描述（s_v）相对于父节点的描述（s_parent）和支持证据是被蕴含、矛盾还是中性。基于LLM的验证器（f_LLM）进一步提炼模糊案例。这确保了已识别演化关系的语义健全性和高保真度，构成了THE-Tree可验证性的支柱。

% The following figure contains the algorithms. It is placed here to follow the flow of text.
\begin{figure*}[h]
    \begin{minipage}[t]{0.49\linewidth}
        \centering
        \begin{algorithm}[H]
        \caption{SGT-MCTS Implementation}
        \label{alg:sgt_mcts}
        \scriptsize
        \begin{algorithmic}[1]
        \Require Root node representing the starting technology concept
        \Ensure Comprehensive technology evolution tree
        \State Initialize the tree with the root node
        \While{not converged}
            \State \textbf{Select:} Choose promising node
            \State \quad node $\gets$ select(root) \Comment{SGT-UCT scoring {\color{blue}(Eq.~\ref{eq:sgt_uct})}}
            \State \textbf{Expand:} Generate new technology nodes
            \State \quad new\_nodes $\gets$ expand(node) \Comment{TVCV methodology {\color{blue}(Alg.~\ref{alg:tvcv_expansion}, Sec.~\ref{sec:auto_construction_tvcv})}}
            \State \textbf{Simulate:} Evaluate potential paths
            \State \quad reward $\gets$ simulate(new\_nodes) \Comment{Sample-based evaluation}
            \State \textbf{Backpropagate:} Update statistics
            \State \quad backpropagate(node, reward) \Comment{Improve future selection}
        \EndWhile
  \State
        \State \Return Constructed technology tree
        \end{algorithmic}
        \end{algorithm}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.49\linewidth}
        \centering
        \begin{algorithm}[H]
\caption{TVCV Node Expansion}
\label{alg:tvcv_expansion}
        \scriptsize
\begin{algorithmic}[1]
\Require{Path history, domain knowledge}
\Ensure{Validated technology node}
\State \textbf{Think:} Generate candidate technology $T$ using LLM
\State $T \sim P_{\text{LLM}}(\cdot \mid \text{Path}, \text{domain knowledge})$
\State \textbf{Verbalize:} Summarize into concise statement
\State $s_v \gets \text{Summarize}(T)$
\State \textbf{Cite:} Retrieve supporting documents
\State $D \gets \text{Retrieve}(s_v)$
\State \textbf{Validate:} Verify logical and temporal coherence
\State $\text{Validate}(s_v, D) = \text{RA-NLI}(s_v, D) \land \text{TemporalCheck}(D)$ \Comment{{\color{blue}RA-NLI detailed in Sec.~\ref{sec:auto_construction_ranli}}}
        \If{Validation successful} \State \Return validated node
\Else
    \State Reject and restart expansion
\EndIf
\end{algorithmic}
\end{algorithm}
    \end{minipage}
\end{figure*}
% Figure for RA-NLI process


% Removed original section 3.7 content as it's integrated into 3.2.4
% Removed original subsection Dynamic Optimization as it's briefly mentioned in 3.2.2
% Removed original subsection The Think-Verbalize-Cite Methodology as it's now 3.2.3
% Removed original subsection Implementation Details as SGT-MCTS algorithm is now part of 3.2.2 and TVCV is 3.2.3
% Removed original subsection Core Algorithm and Theoretical Framework as its content is now under 3.1 and 3.2.2


